Panoptic: the perpetual, oracle-free options protocol

Panoptic is the perpetual, oracle-free, instant-settlement options trading protocol on the Ethereum blockchain. Panoptic enables the permissionless trading of options on top of any asset pool in the Uniswap v3 ecosystem and seeks to develop a trustless, permissionless, and composable options product, i.e., do for decentralized options markets what x*y=k automated market maker protocols did for spot trading.

==> features.tex <==
This section highlights some of the key design principles and features of Panoptic. 

\subsection{Governance minimization}
Panoptic aimed at zero governance, i.e., no parameter should be based on governance decisions but function in a free manner.

\subsection{Gas optimization} To minimize gas consumption, Panoptic will take the following measurements:
\begin{itemize}
    \item not issuing ERC20 tokens by default;
    \item batching liquidity movements; 
    \item deploying liquidity directly on Uni v3 (i.e., no NFT needed);
    \item use IOUs when removing liquidity;
    \item mint options on layer 2, relocate liquidity on layer 1;
    \item incentivize MMs to deploy to a fixed strike interval ($>1\%$).
\end{itemize} 
\subsection{Permissionless listing}
A factory contract can be permissionlessly deployed on top of any Uni v3 pool. The core smart contract will handle the minting of long+short options and market making activity. The deployment of a new option will also require a small amount of funds to be locked in a NFT or staker contract as a way to track pricing (see Section IV.D).


\subsection{Trustless option creation}
The role of the option smart contract is to manage the liquidity on top of the Uni v3 pool smart contract. As such, options are not traded/exchanged between users, rather bought from and sold to Panoptic. Therefore, as long as liquidity is present in a pool and LP locked funds inside Panoptic staker contract, options can be bought/sold.

In addition, while long and short options could be withdrawn from the smart contract as an ERC20 token, the protocol will not mint ERC20 tokens by default to decrease gas fees. Indeed, since options do not expire, most options will either be exercised (if ITM) or closed (if OTM), and they will never need to leave the option smart contract.

\subsection{Capital Efficiency}
Since the creation of spread options positions caps both the profits and losses, users could in theory deploy a position with only a fraction of the capital required to cover the actual price of the underlying asset.

